Leveraging Visual Question Answering for Image-Caption Ranking

Visual Question Answering (VQA) is the task of taking as input an image and a free-form natural language question about the image, and producing an accurate answer. In this work we view VQA as a "feature extraction" module to extract image and caption representations. We employ these representations for the task of image-caption ranking. Each feature dimension captures (imagines) whether a fact (question-answer pair) could plausibly be true for the image and caption. This allows the model to interpret images and captions from a wide variety of perspectives. We propose score-level and representation-level fusion models to incorporate VQA knowledge in an existing state-of-the-art VQA-agnostic image-caption ranking model. We find that incorporating and reasoning about consistency between images and captions significantly improves performance. Concretely, our model improves state-of-the-art on caption retrieval by 7.1% and on image retrieval by 4.4% on the MSCOCO dataset.

==> paper/A04-Interpretability.tex <==



\section{Information of $(Q,A)$ pairs}

Given an image $I$, we propose to rank a set of $N$ candidate $(Q,A)$ pairs by how informative their validity $V_1, V_2,\dots, V_N\in \{ true, false\}$ is to selecting a caption $C$ for image $I$ from a set of $K$ captions $\{ C_1, C_2, \dots C_K\}$. 

We this information with mutual information $MI(V_i;C)$ between the validity $V_i$ of the $i$-th $(Q,A)$ pair $(Q_i, A_i)$ and the caption $C$. By the definition of mutual information

\begin{equation}
MI(V_i;C)=\sum_{v\in\{true,false\}}{\sum_{k}{P(V_i=v,C=C_k) \log \frac{P(V_i=v,C=C_k)}{P(V_i=v)P(C=C_k)}}}
\label{eq:mi}
\end{equation}

In order to compute mutual information we need the following three probabilities.
\begin{itemize}

\item{$P(V_i=v)$:} how likely $(Q_i, A_i)$ is true (valid) or false (invalid) given $I$. We compute that using the prediction from the VQA model. 
%\footnote{Ideally this should be $P(Q_i,A_i|I) = P(A_i|Q_i,I)P(Q_i|I)$, but we assume $P(Q_i|I)$ is 1. Contemporary work~\cite{Ray_2016} has looked at modeling $P(Q_i|I)$, and can be incorporated in our approach.}

\begin{equation}
\begin{aligned}
& P(V_i=true)=P(A_i|Q_i,I)~ \\
& P(V_i=false)=1-P(A_i|Q_i,I)
\end{aligned}
\end{equation}

\item{$P(C=C_k)$:} how likely $C_k$ is the chosen caption of $I$. We compute that using the prediction from our image-caption ranking model.
\begin{equation}
\begin{aligned}
& P(C=C_k)=P_{cap}(C_k|I)
\end{aligned}
\end{equation}

\item{$P(V_i=v,C=C_k)$:} the joint probability of the validity of $(Q_i, A_i)$ and caption $C$. 

Computing the joint probability is an interesting problem. The proposed fusion model is purely feed-forward, so once we have hidden layer activations, the validity of a $(Q,A)$ pair and the caption $C$ are independent. In other words, once we learn a fusion model and feed in the input image/captions/$(Q,A)$ pairs, the hidden layer activations are already determined, and then $V_i$ and $C$ are independently predicted. 

But does that imply $V_i$ and $C$ are independent? No. Because their independence is \emph{conditioned} on the fusion model. From a bayesian perspective, computing the joint probability of $V_i$ and $C$ properly would require marginalizing over the fusion model parameters. 

Let $\Theta$ be the parameters of the fusion model (includes parameters for both VQA and image captioning). We rewrite the joint probablity $P(V_i=v,C=C_k)$ as taking expectation over fusion model parameters $\Theta$ to marginalize it out:

\begin{equation}
\begin{aligned}
& P(V_i=v,C=C_k)=\mathbb{E}_{\theta\sim P(\Theta)}{P(V_i=v,C=C_k|\Theta=\theta)}
\end{aligned}
\end{equation}

Given model parameters, the hidden layer activations are determined and the model would independently predict $V_i$ and $C$. So we assume that $V_i$ and $C$ are indpendent given fusion model parameters $\Theta$. Therefore

\begin{equation}
\begin{aligned}
\label{eq:expectation}
 & P(V_i=v,C=C_k) \\
 &=\mathbb{E}_{\theta\sim P(\Theta)}{P(V_i=v,C=C_k|\Theta=\theta)} \\
 &=\mathbb{E}_{\theta\sim P(\Theta)}{P(V_i=v|\Theta=\theta)P(C=C_k|\Theta=\theta)} \\
 &=\begin{cases}
 \mathbb{E}_{\theta\sim P(\Theta)}{P(A_i|Q_i,I,\theta)P_{cap}(C_k|I,\theta)}&, v=true \\
 \mathbb{E}_{\theta\sim P(\Theta)}{(1-P(A_i|Q_i,I,\theta))P_{cap}(C_k|I,\theta)}&, v=false
\end{cases}
\end{aligned}
\end{equation}


Marginalizing over all possible model parameters is an intractable task. However recent progress on variational methods for neural networks allows us to compute an approximation. Previous works~\cite{Gal_2015,Blundell_2015} have established a theoretical fundation that setting dropout layers in neural networks to training mode at test time can be interpreted as sampling from a variational approximation to the posterior model parameter distribution $P(\Theta)$. They also showed that the dropout distribution can be leveraged to approximately compute model uncertainty. In this work we follow the same framework but instead use dropout to approximate joint probability and mutual information. 

We compute a monte carlo approximation of Eq.~\ref{eq:expectation} by sampling $\theta$ from the dropout distribution as $P(\Theta)$. Specifically, we 

1) Sample model parameters $\theta$ by setting dropout to training mode;

2) Use the same $\theta$ to make both VQA and image-caption ranking predictions; 

3) Average over $\theta$ samples to approximate joint probability $P(V_i=v,C=C_k)$. 

To our knowledge this is the first study on using dropout to compute joint probability and mutual information between two tasks.

\end{itemize}

After the three probabilities are computed, they then go into Eq.~\ref{eq:mi} to compute mutual information between $(Q_i,A_i)$ and caption $C$. And then, the $(Q_i, A_i)$ pair that is selected is the most informative one for a given image I in terms of determining which caption is the best match for the image.

In our experiments, image $I$ is randomly selected from the image-caption ranking test set and we use all its $K=1,000$ candidate captions as $\{ C_1, C_2, \dots C_K\}$. We select the $(Q,A)$ with the highest mutual information from $N=3,000$ $(Q,A)$ pairs randomly selected from VQA training set. We draw $5,000$ dropout samples of $\theta$ to approximately compute mutual information. Qualitative examples of selected (Q,I) pairs for examples images is shown in Figure.5 in the main paper. Our implementation will be publicly available.
